Recognizing Activities of Daily Living with a Wrist-mounted Camera

We present a novel dataset and a novel algorithm for recognizing activities of daily living (ADL) from a first-person wearable camera. Handled objects are crucially important for egocentric ADL recognition. For specific examination of objects related to users' actions separately from other objects in an environment, many previous works have addressed the detection of handled objects in images captured from head-mounted and chest-mounted cameras. Nevertheless, detecting handled objects is not always easy because they tend to appear small in images. They can be occluded by a user's body. As described herein, we mount a camera on a user's wrist. A wrist-mounted camera can capture handled objects at a large scale, and thus it enables us to skip object detection process. To compare a wrist-mounted camera and a head-mounted camera, we also develop a novel and publicly available dataset that includes videos and annotations of daily activities captured simultaneously by both cameras. Additionally, we propose a discriminative video representation that retains spatial and temporal information after encoding frame descriptors extracted by Convolutional Neural Networks (CNN).

==> Makefile <==
.SUFFIXES: .tex .dvi .aux .log .toc .lof .lot .pdf .ps .bbl .bib .blg
F=egpaper_for_review
TEX=platex
CHAPTER=$(shell ls *.tex)
CHAPAUX=$(shell ls *.aux)

all: $F.dvi

pdf: $F.pdf
dvi: $F.dvi
bbl: $F.bbl
ps:  $F.ps

$F.dvi:$F.tex $F.bbl $(CHAPTER)
#$F.dvi:$F.tex $(CHAPTER)
$F.pdf:$F.dvi
$F.ps:$F.dvi
$F.bbl:$F.bib
$F.aux:$F.tex

.dvi.ps:
#	dvips -t a4 -Ppdf -o $@ $*
	dvips -Ppdf -o $@ $*
.dvi.pdf:
	dvipdfmx $*
#	pdflatex -shell-escape $F.tex

.bib.bbl:
	${TEX} $*; pbibtex $*; platex $*; platex $*;

.tex.aux:
	$(TEX) $*

clean:
	rm -f *~ $F.dvi $F.aux $F.lof $F.toc $F.lot $F.log \
               $F.pdf $F.ps $F.bbl $F.blg
	rm -f $(CHAPAUX) *.pbm

